DEF: Deep Estimation of Sharp Geometric Features in 3D Shapes

We propose Deep Estimators of Features (DEFs), a learning-based framework for predicting sharp geometric features in sampled 3D shapes. Differently from existing data-driven methods, which reduce this problem to feature classification, we propose to regress a scalar field representing the distance from point samples to the closest feature line on local patches. Our approach is the first that scales to massive point clouds by fusing distance-to-feature estimates obtained on individual patches. We extensively evaluate our approach against related state-of-the-art methods on newly proposed synthetic and real-world 3D CAD model benchmarks. Our approach not only outperforms these (with improvements in Recall and False Positives Rates), but generalizes to real-world scans after training our model on synthetic data and fine-tuning it on a small dataset of scanned data. We demonstrate a downstream application, where we reconstruct an explicit representation of straight and curved sharp feature lines from range scan data.

==> src/figures/fig_experiments_noise_robustness.tex <==
\begin{figure*}
\centering
\includegraphics[width=\columnwidth]{img/images_synthetic_patches_noise.pdf}
\includegraphics[width=\columnwidth]{img/points_synthetic_patches_noise.pdf}
\caption{DEF is significantly more robust to acquisition noise, compared to other approaches.
This is valid for both image-based (the two left plots, square markers) and point-based (the two right plots, round markers) datasets.
\DZ{critical:perhaps move all data for the point based approach to an appendix, otherwise the main message is muddled. Only DEF-Points vs DEF-Images direct comparisons are needed.
The sharp downturn in the curves for higher noise values need to be explained in the text -- FPR and Recall both go down a lot.
}
}
\label{fig:noise_robustness}
\end{figure*}


==> src/figures/fig_experiments_resolution_robustness.tex <==
\begin{figure*}
\centering
\includegraphics[width=\columnwidth]{img/images_synthetic_patches_resolution.pdf}
\includegraphics[width=\columnwidth]{img/points_synthetic_patches_resolution.pdf}
\caption{Compared to the baseline approaches, DEF is
robust to feature sampling density.
This is valid for both image-based (the two left plots, square markers) and point-based (the two right plots, round markers) datasets.}
\label{fig:resolution_robustness}
\end{figure*}

==> src/tables/tab_synthetic_point_patches.tex <==



\begingroup
\tabcolsep=4pt
\def\arraystretch{1.075}

\begin{table*}[]
\centering
\caption{
Our \emph{local patch-based} deep networks for \emph{distance-to-feature estimation} and feature line \emph{segmentation} are more effective compared to competitor methods across a variety of segmentation and regression quality measures.}
\resizebox{0.995\textwidth}{!}{%
\begin{tabular}{@{}lccccclcccc@{}}
\toprule
 &
  \multicolumn{4}{c}{Synthetic image patches, $n = 50$ ($r = 0.02$)} &
   &
   &
  \multicolumn{4}{c}{Synthetic point patches, $n = 50$ ($r = 0.02$)} \\ \cmidrule(lr){2-5} \cmidrule(l){8-11} 
Method & 
  \rmse$\downarrow$   & 
  \qrmse$\downarrow$   & 
  \recall$(1r)$, \%$\uparrow$   & 
  \fpr$(1r)$, \%$\downarrow$ &  & 
Method & 
  \rmse$\downarrow$   & 
  \qrmse$\downarrow$   & 
  \recall$(1r)$, \%$\uparrow$   & 
  \fpr$(1r)$, \%$\downarrow$ \\
   & $\times 10^{-3}$ & $\times 10^{-3}$ & &  
 & & & $\times 10^{-3}$ & $\times 10^{-3}$ & & 
\\ \cmidrule(r){1-5} \cmidrule(l){7-11} 
VCM~\cite{merigot2010voronoi} & --- &  ---  & 49.1 & 3.1 &  & 
VCM~\cite{merigot2010voronoi} & --- &  ---  & 90.4 & 2.3 \\
EC-Net~\cite{yu2018ec}        & --- &  ---  & 79.2 & 2.9 &  & 
EC-Net~\cite{yu2018ec}        & --- &  ---  & 85.4 & 1.9 \\
PIE-NET~\cite{wang2020pie}    & --- &  ---  & 32.0 & 3.8 &  & 
PIE-NET~\cite{wang2020pie}    & --- &  ---  & 16.3 & 2.2 \\
ShF~\cite{raina2019sharpness} & 18.0 & 95.7 & 80.9 & 0.3 &  & 
ShF~\cite{raina2019sharpness} & 59.5 & 167.7 & \textbf{94.1} & 3.5 \\
\cmidrule(r){1-5} \cmidrule(l){7-11} 
DEF-Image (Ours)     & 
  11.1  & 
  42.5 & 
  80.0 & 
  $\mathbf{2.2\times 10^{-2}}$  &
   &
   DEF-Points (Ours)  & 
  10.0  & 
  38.1 & 
  89.5 & 
  $\mathbf{7 \times 10^{-2}}$ \\
 DEF-Image-nobg (Ours) &
  \textbf{9.7} &
  \textbf{32.5} &
  \textbf{84.6} &
  $3 \times 10^{-2}$ &  
  & 
 DEF-Points + VCM (Ours)    & 
  \textbf{7.8} & 
  \textbf{25.6} & 
  90.0 & 
  $8 \times 10^{-2}$\\
 
DEF-Points (Ours) &
  11.3 &
  55.5 &
  80.9 &
  $3.7 \times 10^{-2}$
  & & & & &  
  & \\
\bottomrule
\end{tabular}
}

\label{tab:synthetic_patches}
\end{table*}

\endgroup
